Strong and fast rising pressure waves emitted by plasmonic vapor nanobubbles

Plasmonic vapour nanobubbles are currently considered for a wide variety of applications ranging from solar energy harvesting and photoacoustic imaging to nanoparticle-assisted cancer therapy. Yet, due their small size and unstable nature, their generation and consequences remain difficult to characterize. Here, building on a phase-field model, we report on the existence of strong pressure waves that are emitted when vapor nanobubbles first form around a laser-heated nanoparticle immersed in water, and subsequently after bubble rebound. These effects are strongest when the fluid is locally brought high in its supercritical state, which may be realized with a short laser pulse. Because of the highly out-of-equilibrium nature of nanobubble generation, the waves combine a high pressure peak with a fast pressure rising time, and propagate in water over micron distances, opening the way to induce spatially and temporally localized damage. Discussing the consequences on biological cell membranes, we conclude that acoustic-mediated perforation is more efficient than nanobubble expansion to breach membrane. Our findings should serve as guide for optimizing the thermoacoustic conversion efficiency of plasmonic vapor nanobubbles.

==> Acoustics_2020-macros.tex <==
\usepackage{color}
%\newcommand{\cm}[1]{{\color{blue} #1}}
%\newcommand{\jl}[1]{\textcolor{blue}{{#1}}}

\newcommand{\cm}[1]{#1}
\newcommand{\jl}[1]{#1}


\usepackage{pifont} %dingbat symbol


% Macros for notations
\newcommand{\dawsonmax}{F_\xam^D}
\newcommand{\dPdTrho}{\left(\frac{\partial P}{\partial T}\right)_{\!\!\!\rho_0}}  
%\newcommand{\deltaTnpnoloss}{\Delta \Tnp^{\rm no \ loss}}
\newcommand{\deltaTnpnoloss}{\Delta \Tnp^*}
\newcommand{\ea}{e_{\rm a}}
\newcommand{\Ea}{E_{\rm a}}
\newcommand{\Ef}{E_{\rm f}}
\newcommand{\EL}{E_{\rm L}}
\newcommand{\Esigma}{E_\gamma}
\newcommand{\ga}{{\gamma}}
\newcommand{\Fth} {F_\mathrm{th}}
\newcommand{\nth}{n^{\rm th}}
\newcommand{\Pmax}{P_{\rm max}}
\newcommand{\Pprime}{P'}
\newcommand{\tauep}{\tau_\mathrm{ep}}
\newcommand{\tauk}{\tau_\mathrm{K}}
%\newcommand{\tp}{\tau_\mathrm{p}}
\newcommand{\tvap}{t_\mathrm{vap}}
\newcommand{\taup}{\tau_\mathrm{p}}
\newcommand{\taur}{\tau_\mathrm{r}}
\newcommand{\Tmax}{T_\xam}
\newcommand{\To}{T_0}
\newcommand{\Ts}{T_\mathrm{s}}
\newcommand{\Tsp}{T_\mathrm{sp}}
\newcommand{\xam}{\mathrm{max}}

% fluid
%\newcommand{\cf} {C_\mathrm{f}}
\newcommand{\cf} {C}
%\newcommand{\lamf} {\lambda_\mathrm{f}}
\newcommand{\lamf} {k}

\newcommand{\cnp}{C_\mathrm{np}}
\newcommand{\Rnp}{R_\mathrm{np}}
\newcommand{\signp}{\sigma_\mathrm{abs}}
\newcommand{\Snp}{S_\mathrm{np}}
\newcommand{\Tnp}{T_\mathrm{np}}
\newcommand{\Vnp}{V_\mathrm{np}}

%\vectors
\newcommand{\vcr}{\mathbf{r}}
\newcommand{\vv}{\mathbf{v}}

%\SM macros
\newcommand{\flap}{\mathcal{F}}

\newcommand{\fnp } {f_\mathrm{np}}
\newcommand{\fmeds}{f_\mathrm{s}}
\newcommand{\fmed }{f}

\newcommand{\ftilde}  {\tilde{f}}
\newcommand{\fnptilde}{\ftilde_\mathrm{np}}
\newcommand{\fmedstilde}{\ftilde_\mathrm{s}}



%%% not used so far

%\usepackage{graphicx,color,ifthen}
%\usepackage{pstricks,pst-node,pst-text,pst-3d,color}
%\usepackage[notref]{showkeys}
%\usepackage{times}


%\setlength{\textheight}{23.5cm}
%%\setlength{\columnwidth}{82mm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parskip}{0cm}

